On the Convergence Theory of Gradient-Based Model-Agnostic Meta-Learning Algorithms

We study the convergence of a class of gradient-based Model-Agnostic Meta-Learning (MAML) methods and characterize their overall complexity as well as their best achievable accuracy in terms of gradient norm for nonconvex loss functions. We start with the MAML method and its first-order approximation (FO-MAML) and highlight the challenges that emerge in their analysis. By overcoming these challenges not only we provide the first theoretical guarantees for MAML and FO-MAML in nonconvex settings, but also we answer some of the unanswered questions for the implementation of these algorithms including how to choose their learning rate and the batch size for both tasks and datasets corresponding to tasks. In particular, we show that MAML can find an $\epsilon$-first-order stationary point ($\epsilon$-FOSP) for any positive $\epsilon$ after at most $\mathcal{O}(1/\epsilon^2)$ iterations at the expense of requiring second-order information. We also show that FO-MAML which ignores the second-order information required in the update of MAML cannot achieve any small desired level of accuracy, i.e., FO-MAML cannot find an $\epsilon$-FOSP for any $\epsilon>0$. We further propose a new variant of the MAML algorithm called Hessian-free MAML which preserves all theoretical guarantees of MAML, without requiring access to second-order information.

==> Final Draft/Conclusion.tex <==
%!TEX root = main.tex

\section{Conclusion}
In this work, we studied the convergence properties of MAML, its first-order approximation (FO-MAML), and our proposed Hessian-free MAML (HF-MAML) for non-convex functions. In particular, we characterized their best achievable accuracy in terms of gradient norm when we have access to enough samples and further showed their best possible accuracy when the number of available samples is limited. Our results indicate that MAML can find an $\eps$-first-order stationary point, for any positive $\eps$ %, while it suffers from an iteration cost of $\bigO(d^2)$. 
{at the cost of using the second-order information of loss functions.}
On the other hand, we illustrated that although the iteration cost of FO-MAML is $ \bigO(d)$, it cannot reach any desired level of accuracy. That said, we next showed that  HF-MAML has the best of both worlds, i.e., it {does not require access to the second-order derivative and} has a cost of $\bigO(d)$ at each iteration, while it can find an $\eps$-first-order stationary point, for any positive $\eps$.


==> Final Draft/Experiments.tex <==
%!TEX root = main.tex

\section{A Numerical Example}\label{Numerical}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% Figure %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure}
   \centering
     \begin{subfigure}[H]{0.45\textwidth}
       \includegraphics[width=1\columnwidth]{Fig_1}
             \subcaption{Having exact gradients \& Hessians available}
       \label{Fig_1}
       \end{subfigure}
       \qquad 
 %%%%%%%%%%%%%%%%%%%
     \begin{subfigure}[H]{0.45\textwidth}
      \includegraphics[width=1\columnwidth]{Fig_2}
       \subcaption{Stochastic gradients \& Hessians with similar tasks}
       \label{Fig_2}
   \end{subfigure}\\
 %%%%%%%%%%%%%%%%%%%   
     \begin{subfigure}[H]{0.45\textwidth}
       \includegraphics[width=1\columnwidth]{Fig_3}
             \subcaption{Stochastic gradients \& Hessians with less similar tasks}
       \label{Fig_3}
       \end{subfigure}
 %%%%%%%%%%%%%%%%%%%
     \caption{Comparison of MAML, FO-MAML, and HF-MAML for a 1-rank matrix factorization problem}\label{Fig_Main} 
  \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We consider a 1-rank matrix factorization problem where the loss for task $i$ is 
\begin{equation*}
f_i(x) = \frac{1}{4} \| x x^\top - M_i \|_F^2	
\end{equation*}
where $\|.\|_F$ is the Frobenius norm, and, $M_i$ is a rank one matrix, generated as $M_i=g_i g_i^\top$ where $g_i$ is a random zero-mean Gaussian vector. The variance of $g_i$ controls task similarity ($\sigma^2$). To capture noisy gradients and Hessians we add random Gaussian noise with variance $\tsigma^2$ to the tasks gradients and Hessians.

Recall from our results that the best accuracy for MAML and HF-MAML is $\bigO(\tilde{\sigma}/\sqrt{D})$ while the one for FO-MAML is $\bigO(\alpha \sigma + \tilde{\sigma}/\sqrt{D})$, which has the additional term $\bigO(\alpha \sigma)$, and hence, it does not go to zero even with exact gradients and Hessians.
\begin{itemize}
\item In Figure \ref{Fig_1}, we assume gradients and Hessians are exact ($\tilde{\sigma}=0$) and focus on task variation. We assume that the batch-size for tasks $B$ equal to the number of tasks which is 20. In this case, even though the gradients are exact, FO-MAML converges to an error level with a gap compared to two others. This is consistent with our results.
\item We next consider noisy gradients and Hessians. We also set $B$=10 and number of tasks equal to 50. In Figure \ref{Fig_2}, we choose the variance of $g_i$ small to ensure the tasks are relatively similar. Here the additional persistent error of FO-MAML is negligible compared to the other term and all three methods behave similarly.
\item In Figure \ref{Fig_3}, we increase the variance of $g_i$, i.e., tasks are less similar. In this case, the $\bigO(\alpha \sigma)$ term dominates the other term in the error of FO-MAML, and it has worse performance compared to two others.
\end{itemize}








==> Final Draft/HFMAML.tex <==
%!TEX root = main.tex

\section{Hessian-free MAML (HF-MAML)}

To reduce the cost of implementing MAML we propose an approximate variant of MAML  that is \textit{Hessian-free}, i.e., only requires evaluation of gradients, and has a computational cost of $\mathcal{O}(d)$. 
The idea behind our method is that for any function $\phi$, the product of Hessian $\nabla^2 \phi (w) $ by a vector $v$ can be approximated by 
%%%%
\begin{equation}
    \nabla^2 \phi (w)  v \approx \left[ 
    \frac{\nabla \phi(w+\delta v)-\nabla \phi(w-\delta v)}{2\delta}\right]
\end{equation}
%%%
with an error of at most $\rho \delta \|v\|^2$, where $\rho $ is the parameter for Lipschitz continuity of the Hessian of $\phi$. Based on this approximation,
% the update in \eqref{method_update} can be interpreted as a Hessian-free approximation of GD for Meta-learning. 
%The update in \eqref{method_update} suggests a 
we propose a computationally efficient approach for %implementing the update of MAML when we aim to 
minimizing the expected loss $F$ defined in \eqref{main_prob}
%Indeed, this idea can be easily extended for implementation of SGD and in particular the MAML algorithm 
which we refer to it as Hessian-free MAML (HF-MAML). As the name suggests the HF-MAML is an approximation of the MAML that does not require evaluation of any Hessian, while it provides an accurate approximation of MAML. To be more precise, the update of HF-MAML is defined as 
%%%
\begin{align}\label{HF_MAML_main_update}
w_{k+1} =  w_k - \frac{\be_k}{B} \sum_{i \in \B_k} \left[\tilde{\nabla} f_i\!\left(w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i\right)  -\alpha  d_k^i \right] 
\end{align}
%%%
where $\alpha$ is the step size for each task, $\beta_k$ is the stepsize for the meta update, and the vectors $d_k^i$ are defined as 
%%%
{\small
\begin{align}\label{d_HF_MAML}
& d_k^i :=  \frac{1}{2\delta_k^i} \left ( \tilde{\nabla} f_i \!\left(w_k\!+\!\delta_k^i \tilde{\nabla} f_i(w_k\!-\!\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i), \D_{h}^i\right) \right. \nonumber \\
& \left. -\!\tilde{\nabla} f_i\!\left(w_k\!-\!\delta_k^i \tilde{\nabla} f_i(w_k\!-\!\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i),\D_{h}^i\right) \right ).
\end{align}}
%%
Note that $d_k^i$ is an approximation for the term $ \tilde{\nabla}^2 f_i(w_{k},\D_{h}^i) \tilde{\nabla} f_i(w_k\!-\!\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i)$ which appears in $\nabla F$. In addition, $\delta_k^i>0$ indicates the accuracy of the Hessian-vector product approximation.  
%As in MAML, this update can be implemented efficiently in two stages where in the first one we compute points $w_{k+1}^i$ by performing the following update %%%
%\begin{equation}\label{inner_step_2}
%w_{k+1}^i = w_k - \al \tilde{\nabla}f_i(w_k,\D_{in}^i)
%\end{equation}
%%%%%
%for all tasks $\T_i\in \B_k$, which is identical to \eqref{inner_step}. Then we use these models in the outer loop to evaluate the vectors $d_k^i$ given in \eqref{d_HF_MAML} %based on the update
%%%%%
%%\begin{align}
%%d_k^i=  \frac{\tilde{\nabla} f_i \left(w_k+\delta_k^i \tilde{\nabla} f_i(w_{k+1}^i,\D_{o}^i), \D_{h}^i\right)-\tilde{\nabla} f_i \left(w_k-\delta_k^i \tilde{\nabla} f_i(w_{k+1}^i,\D_{o}^i),\D_{h}^i\right)}{2\delta_k^i},
%%\end{align}
%%%%
% %where the vector $d_k^i$ 
% which approximates the Hessian-vector product $ \tilde{\nabla}^2 f_i(w_{k},\D_{h}^i)\tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i)$. Then we compute the updated meta model $w_{k+1}$ based on
%%%%
%\begin{align}
%w_{k+1} &= w_k -  \frac{\be_k}{B} \sum_{i \in \B_k} \left(\tilde{\nabla} f_i\!\left(w_{k+1}^i,\D_{o}^i \right) -\alpha d_k^i \right).
%\end{align}
%%%%
%The steps of HF-MAML are outlined in Algorithm~\ref{Algorithm3}.
As depicted in Algorithm~\ref{Algorithm3}, this update can be implemented efficiently in two stages similar to MAML. 
%In our theoretical results we characterize the error induced by the Hessian-vector product approximation and show how one should choose all the parameters of HF-MAML including $B$, $D_{in}$,  $D_o$, $D_h$, $\beta_k$, and $\delta_k^i$.
\begin{algorithm}[t!]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    %\underline{function Euclid} $(a,b)$\;
    %\Input{Initial iterate $w_0$}
	\While{not done}{
    Choose a batch of \textit{i.i.d.} tasks $\B_k \subseteq \I$ with distribution $p$ and with size $B = |\B_k|$;\\
    \For{all $\T_i$ with $i \in \B_k$}{
    Compute  $\tilde{\nabla}f_i(w_k,\D_{in}^i)$ using dataset  $\D_{in}^i$;\\
    Set $w_{k+1}^i = w_k - \al \tilde{\nabla}f_i(w_k,\D_{in}^i)$;\\
    %Set $\tilde{\nabla}F_i(w_{k+1}^i)$ be an unbiased estimate of $\nabla F_i(w_{k+1}^i)$ using batches $\D_o^i, \D_h^i$;\\
    }
%    Compute $\displaystyle{d_k^i=  \frac{\tilde{\nabla} f_i\left(w_k+\delta_k^i \tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i), \D_{h}^i\right)-\tilde{\nabla} f_i\left(w_k-\delta_k^i \tilde{\nabla} f_i(w_{k+1}^i,\D_{o}^i),\D_{h}^i\right)}{2\delta_k^i}}$;\\
%Compute $d_k^i$ given in \eqref{d_HF_MAML}; \\
%    $w_{k+1} \gets w_k - \frac{\be_k}{B} \sum_{i \in \B_k} (\tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i) -\al d_k^i)$; \\
Compute $w_{k+1}$ according to the update \eqref{HF_MAML_main_update}; \\
    $k \gets k + 1$;
    }
    \caption{\label{Algorithm3} Hessian-free MAML (HF-MAML)}
\end{algorithm}

==> Final Draft/Introduction.tex <==
%!TEX root = main.tex



% 

\section{Introduction}
In several artificial intelligence problems, ranging from robotics to image classification and pattern recognition, the goal is to design systems that use prior experience and knowledge to learn new skills more efficiently. \textit{Meta-learning} or \textit{learning to learn} formalizes this goal by using data from previous tasks to learn update rules or model parameters that can be fine-tuned to perform well on new tasks with small amount of data \citep{LearningToLearn}. Recent works have integrated this paradigm with neural networks including learning the initial weights of a neural network \citep{finn17a, Reptile}, updating its architecture \citep{baker2016designing, zoph2016neural, zoph2018learning}, or learning the parameters of optimization algorithms using recurrent neural networks \citep{ravi2016optimization, NIPS2016_Andry}.

A particularly effective approach, proposed in \citep{finn17a}, is the gradient-based meta-learning in which the parameters of the model are explicitly trained such that a small number of gradient steps with a small amount of training data from a new task will produce good generalization performance on that task. This method is referred to as \textit{model-agnostic meta learning (MAML)} since it can be applied to any learning problem that is trained with gradient descent. Several papers have studied the empirical performance of MAML for nonconvex settings \citep{Reptile, MAML++, Meta-SGD, CAVIA, grant2018recasting, alpha-MAML, al-shedivat2018continuous}. However, to the best of our knowledge, its convergence properties have not been established for general non-convex functions.

In this paper, we study the convergence of variants of MAML methods for nonconvex loss functions and establish their computational complexity as well as their best achievable level of accuracy in terms of gradient norm.    
More formally, let $\T = \{\T_i\}_{i \in \I}$ denote the set of all tasks and let $p$ be the probability distribution over tasks $\T$, i.e., task $\T_i$ is drawn with probability $p_i= p(\T_i)$. We represent the loss function corresponding to task $\T_i$ by $f_i(w): \R^d \to \R$ which is parameterized by the same $w \in \R^d$ for all tasks. Here, the loss function $f_i$ measures how well an action $w$ performs on task $\T_i$. The goal of expected risk minimization is to minimize the expected loss over all tasks, i.e., 
%%%
\begin{equation}\label{f_def}
\min f(w) := \E_{i\sim p}[f_i(w)].
\end{equation}
%%%
In most learning applications, the loss function $f_i$ corresponding to task $\T_i$ is defined as an expected loss with respect to the probability distribution which generates data for task $\T_i$, i.e., 
%\begin{equation}\label{f_i_def}
$f_i(w) := \E_{\theta}[f_i(w, \theta)]$.
%\end{equation}
In this case, the gradient and Hessian of $f_i$ can be approximated by $\nabla f_i(w,\D) := \frac{1}{|\D|} \sum_{\theta \in \D} \nabla f_i (w,\theta)$ and $\nabla^2 f_i(w,\D) := \frac{1}{|\D|} \sum_{\theta \in \D} \nabla^2 f_i (w,\theta)$, respectively, where $\D$ is a batch chosen from the dataset of task $\T_i$.  %\sloppy To better highlight this point, as an example, consider a supervised learning problem in which each task $\T_i$ corresponds to the problem of finding weights $w$ of a predictive model $h(w;.)$ such as a deep neural network for predicting the label $y$ of a sample point $x$. In this case, the loss $f_i$ is defined as the population risk ${f_i(w) = \E_{(x,y)}[\ell(w; x,y)]=  \E_{(x,y)}[ \|y-h(w;x)\|^2 ],}$ where $h(w;x)$ is the prediction of $x$'s label given the model $w$ and $\ell$ is the quadratic loss function. Note that for this special case, the stochastic gradient $\tilde{\nabla}f_i(w,\D)$ is given by $\frac{1}{|\D|} \sum_{(x_j,y_j)\in \D} \nabla \ell (w;x_j,y_j)$.

In traditional statistical learning, we solve Problem \eqref{f_def} as we expect its solution to be a proper approximation for the optimal solution of a new unseen task $\T_i$. However, in model-agnostic meta-learning, we aim to find the best point that performs well as an initial point for learning a new task $\T_i$ when \textit{we have budget for running a few steps of gradient descent} \citep{finn17a}. For simplicity, we focus on finding an initialization $w$ such that, after observing a new task $\T_i$, one gradient step would lead to a good approximation for the minimizer of $f_i(w)$. We can formulate this goal as 
%%% 
\begin{equation}\label{main_prob}
\min F(w) := \E_{i \sim p}\left[ F_i(w)\right]
:= \E_{i \sim p}\left[f_i(w - \al \nabla{f_i(w)})\right],
\end{equation}
%%%%
where $\alpha>0$ is the stepsize for the update of gradient descent method and $F_i(w)$ denotes $f_i(w - \al \nabla{f_i(w)})$.

Problem \eqref{main_prob} is defined in a way that its optimal solution would perform well in expectation when we observe a task and look at the output after running a single step of \textit{gradient} descent.\footnote{We only consider the case that one step of gradient is performed for a new task, but, indeed, a more general case is when we perform multiple steps of gradient descent (GD). However, running more steps of GD comes at the cost of computing {multiple Hessians} and for simplicity of our analysis we only focus on a single iteration of GD.} 

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-0.5cm}
\hspace{-2.2cm}  \includegraphics[width=0.75\textwidth]{Fig1_MAML.pdf}
\vspace{-1.5cm}
    \caption{\label{Fig1_MAML} Comparison of the performance of the optimal solution of the statistical learning problem in \eqref{f_def} and the optimal solution of the met-learning problem in \eqref{main_prob} when we have budget for two steps of gradient descent update.}
    \vspace{-0.2cm}
\end{wrapfigure}

However, in most applications, computing the exact gradient for each task is costly and we can only run steps of the stochastic gradient descent (SGD) method. In this case, our goal is to find a point $w$ such that when a task $\T_i$ is chosen, after running one step of SGD, the resulting solution performs well in expectation. In particular, we assume we have access to the stochastic gradient $\tilde{\nabla} f_i(w,\D^i_{test})$ which is an unbiased estimator of $\nabla f_{i}(w)$ evaluated using the batch $\D^i_{test}$ with size $D_{test}$. In this formulation, our goal would change to solving the problem
%%% 
\begin{equation}\label{main_prob_2}
\min \hat{F}(w)
:=\E_{i \sim p}\left[\E_{\D^{i}_{test}} \left[ f_i(w - \al \tilde{\nabla} f_i(w,\D^i_{test}))\right] \right],
\end{equation}
%%%%
where the expectation is taken with respect to selection of task $i$ as well as selection of random set $\D^i_{test}$ for computing stochastic gradient. Throughout the paper, we will clarify the connection between $F$ and $\hat{F}$, and we report our results for both of these functions.
 
It is worth emphasizing that the solution of the standard expected risk minimization in \eqref{f_def} gives us the best answer when we are given many tasks and we plan to choose only ``one action'' that  performs well in expectation, when we observe a new unseen task. On the other hand, the solution of the expected risk minimization in \eqref{main_prob} is designed for the case that we have access to a large number of tasks and we aim to choose ``an action that after one or more steps of gradient descent'' performs well for an unseen task. In the first case, we naturally choose an action that is closer to the optimal solutions of the tasks that have higher probability, but in the second case we choose an action that is closer to the optimal solutions of the tasks that have higher probability and are harder for gradient descent to solve them. For instance, when the loss functions are strongly convex and smooth, a harder task (minimization problem) for gradient descent is the problem that has a larger condition number. Therefore, the solution of \eqref{main_prob} is naturally closer to the solution of those tasks that have larger condition numbers. 

To better highlight the difference between the solutions of the statistical learning problem in~\eqref{f_def} and the meta-learning problem in~\eqref{main_prob}, we consider an example where we have access to three equally likely tasks $\T_1$, $\T_2$, and $\T_3$ with the optimal solutions $w_{*}^{\T_1}$, $w_{*}^{\T_2}$, $w_{*}^{\T_3}$, respectively; see Figure \ref{Fig1_MAML}. Here, $w$ is the solution of Problem~\eqref{f_def} and $\hat{w}$ is the solution of Problem~\eqref{main_prob}. %For simplicity assume that the probability of the three tasks are equal. In this case, $w$ is the best action in expectation with respect to all the observed tasks and $\hat{w} is the best solution in expectation with respect to all the observed tasks when we measure the error after performing two steps of gradient descent. 
In this example, task $\T_1$ is the easiest task as we can make a lot of progress with only two steps of GD and  task $\T_2$ is the hardest task as we approach the optimal solution slowly by taking gradient steps. As we observe in Figure~\ref{Fig1_MAML}, for task $\T_3$, if we start from $w$ the outcome after running two steps of GD is almost the same as starting from $\hat{w}$. For task $\T_1$, however, $w$ is a better initial point compared to $\hat{w}$, but the error of their resulting solution after two steps of GD are not significantly different. This is due to the fact that $\T_1$ is easy and for both cases we get very close to the optimal solution even after two steps of GD.  The difference between starting from $w$ and $\hat{w}$ is substantial when we aim to solve task $\T_2$ which is the hardest task. Because of this difference, the updated variable after running two steps of GD has a lower expected error when we start from $\hat{w}$ comparing to the case that we start from $w$. This simple example illustrates the fact that if we know a-priori that after choosing an model we are allowed to run a single (or more) iteration of GD to learn a new task, then it is better to start from the minimizer of \eqref{main_prob} rather than the minimizer of~\eqref{f_def}.

%%%%
%\begin{figure}[t!]
%\includegraphics[width=0.5\textwidth]{Fig1_MAML.pdf}
%    \caption{\label{Fig1_MAML} Comparing problems \eqref{f_def} and \eqref{main_prob}} %the optimal solution of the statistical learning problem in \eqref{f_def} and the optimal solution of the met-learning problem in \eqref{main_prob} when we have a budget for two steps of gradient descent update.}
%\end{figure}
%%%%

\begin{table*}[t!]
\footnotesize
%\vskip 0.1in
%\caption{Summary of our result} \label{table-1}
\begin{center}
\begin{tabular}{ |l|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Algorithm}}&  \multicolumn{4}{c|}{\textbf{Having access to sufficient samples}} & {\textbf{K-shot Learning}} \\

 & Best accuracy & Iteration & \# samples/ & Runtime/ & Best accuracy\\ 
 & possible & complexity & iteration & iteration & possible\\
 %& \\
\hline
\multirow{2}{*}{\textbf{MAML}} & \multirow{2}{*}{$\| \nabla F(w) \| \leq \eps$} & \multirow{2}{*}{$\bigO(1/\eps^2)$} & \multirow{2}{*}{$\bigO(1/\eps^4)$} & \multirow{2}{*}{$\bm{\bigO(d^2)}$} & \multirow{2}{*}{$\| \nabla F(w) \| \leq \bigO(\tsigma/\sqrt{K})$} \\
 & & & & &\\
\hline
\multirow{2}{*}{\textbf{FO-MAML}} & \multirow{2}{*}{$\| \nabla F(w) \| \leq \bm{\bigO(\alpha \sigma)}$} & \multirow{2}{*}{$\bigO(1/(\alpha^2 \sigma^2))$} & \multirow{2}{*}{$\bigO(1/(\alpha^4 \sigma^2))$} & \multirow{2}{*}{$\bigO(d)$} & \multirow{2}{*}{$\| \nabla F(w) \| \leq \bigO(\bm{\sigma}+ \tsigma/\sqrt{K})$} \\
 & & & & &\\
\hline
\multirow{2}{*}{\textbf{HF-MAML} } & \multirow{2}{*}{$\| \nabla F(w) \| \leq \eps$} & \multirow{2}{*}{$\bigO(1/\eps^2)$} & \multirow{2}{*}{$\bigO(1/\eps^4)$} & \multirow{2}{*}{${\bigO(d)}$} & \multirow{2}{*}{$\| \nabla F(w) \| \leq \bigO(\tsigma/\sqrt{K})$} \\
& & & & &\\
\hline
\end{tabular}
\end{center}
\caption{\label{table-1}Our theoretical results for convergence of MAML, first-order approximation of MAML (FO-MAML), and our proposed Hessian-free MAML (HF-MAML) to a first-order stationary point (FOSP) in nonconvex settings. Here, $d$ is the problem dimension, $\sigma$ is a bound on the standard deviation of $\nabla f_i(w)$ from its mean $\nabla f(w)$, and $\tsigma$ is a bound on the standard deviation of $\nabla f_i(w. \theta)$, an unbiased estimate of $\nabla f_i(w)$, from its mean $\nabla f_i(w)$, for every $i$. For any $\eps>0$, MAML can find an $\eps$-FOSP, while each iteration has a complexity of $\mathcal{O}(d^2)$. FO-MAML has a lower complexity of $\mathcal{O}(d)$, but it cannot reach a point with gradient norm less than $\mathcal{O}(\alpha \sigma)$. HF-MAML has the best of both worlds, i.e., HF-MAML has a cost of $\mathcal{O}(d)$, and it can find an $\eps$-FOSP for any $\eps>0$.}
\end{table*}%
%{} 


\subsection{Our contributions}

 In this paper, we provide the first theoretical guarantees for the convergence of MAML algorithms to first order stationarity for \textit{non-convex} functions. We build our analysis upon interpreting MAML as a SGD method that solves Problem \eqref{main_prob} while we show the analysis of MAML is significantly more challenging due to various reasons, including unbounded smoothness parameter and the biased estimator of gradient used in the update rule of MAML. 
Overcoming these challenges, we characterize the iteration and sample complexity of MAML method and shed light on the relation of batch sizes and parameters of MAML with its convergence rate and accuracy. Using these results, we provide an explicit approach for tuning the hyper-parameters of MAML and also the required amount of data to reach a first-order stationary point of \eqref{main_prob}. A summary of the results\footnote{We assume $\sigma$ and $\tsigma$ are small for the results in this section. The general result can be found in Section \ref{sec:Theory}.} and the specific case of $K$-shot learning, where for each task in the inner loop we have access to $K$ samples, is provided in Table \ref{table-1}. Note that in these results, $\sigma$ is a bound on the standard deviation of $\nabla f_i(w)$ from its mean $\nabla f(w)$, and $\tsigma$ is a bound on the standard deviation of $\nabla f_i(w. \theta)$ from its mean $\nabla f_i(w)$, for every $i$. For formal definitions of $\sigma$ and $\tsigma$ please check Assumptions \ref{asm_bounded_var} and \ref{asm_bounded_var_i}, respectively.

%Specifically, we show MAML finds an $\epsilon$-first-order stationary point ($\epsilon$-FOSP) of Problmes \eqref{main_prob} and \eqref{main_prob_2} after at most $\mathcal{O}(1/\epsilon^2)$ iterations and $\mathcal{O}(1/\epsilon^4)$ stochastic gradient evaluations per iteration, while the complexity of each iteration is of $\mathcal{O}(d^2)$. Our result also directly applies to the specific case of $K$-shot learning where for each task in the inner loop we only have access to $K$ samples. In this case, MAML finds a solution $w_{KS}$ such that $\| \nabla F(w_{KS}) \| \leq \bigO(\sqrt{\tsigma^2/K})$ \footnote{We assume $\sigma$ and $\tsigma$ are small for the results in this section. The general result can be found in Section \ref{sec:Theory}.} where $\tsigma^2$ denotes the bound on the variance of stochastic gradient of $\nabla f_i(w)$ (see Assumption \ref{asm_bounded_var_i} for the precise definition).

As described in \citep{finn17a}, the implementation of MAML is costly\footnote{The cost per iteration is $\bigO(d^2)$ in general. However, it is worth noting that  this cost reduces to $\bigO(d)$ for the case of neural network classifiers using back propagation.} as it requires Hessian-vector product computation. To resolve this issue, \cite{finn17a} suggest ignoring the second-order term in the update of MAML and show that the first-order approximation does not affect the performance of MAML in practice. In our work, we formally characterize the convergence results for this first-order approximation of MAML (\textit{FO-MAML}) and show that if the learning rate $\alpha$ used for updating each task is small or the tasks are statistically close to each other, then the error induced by the first-order approximation is negligible (see Table \ref{table-1}). 
%Specifically, we show that, when we have access to sufficient samples, FO-MAML finds a point $w^\dag$ such that $\| \nabla F(w^\dag) \| \leq \bigO(\alpha \sigma)$ in $\bigO(1/(\alpha^2 \sigma^2))$ iterations. Hence, when $\alpha$ or $\sigma$ are small enough such that $\alpha \sigma = \bigO(\eps)$ we do not lose that much by ignoring the second term, i.e., we can find a point with its gradient norm of $\bigO(\eps)$. 
Nevertheless, in general, in contrast to MAML which can find an $\eps$-first order stationary point for any $\eps>0$, FO-MAML is limited to $\eps \geq \bigO(\alpha \sigma)$.

 To address this issue, we introduce a new method, \textit{Hessian-free MAML (HF-MAML)}, which recovers the complexity bounds of MAML without access to second-order information and has a computational complexity of $\mathcal{O}(d)$ per iteration (see Table \ref{table-1}). In fact, we show that,
  %HF-MAML enjoys a better convergence rate in comparison to FO-MAML, and, 
  for any positive $\eps$, HF-MAML finds an $\epsilon$-FOSP
  % after $\mathcal{O}(1/\epsilon^2)$ iterations 
  while keeping the computational cost $\bigO(d)$ at each iteration. {Hence, HF-MAML has the best of both worlds: it has the low computational complexity of FO-MAML and it achieves any arbitrary accuracy for first-order stationarity as in MAML.} %A summary of our results is provided in Table \ref{table-1}.
  

==> Final Draft/MAML.tex <==
%!TEX root = main.tex
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{MAML Algorithm}\label{sec:MAML}


The MAML algorithm was proposed in \citep{finn17a} for solving the stochastic optimization problem in \eqref{main_prob}. In MAML, at each step $k$, we choose a subset  $\mathcal{B}_k$  of the tasks, with each task drawn independently from distribution $p$. For simplicity assume that the size of $\mathcal{B}_k$ is fixed and equal to $B$. Then, the update of MAML is implemented at two levels: (i) inner step and (ii) outer step (meta-step).

\setlength{\textfloatsep}{4pt}% Remove \textfloatsep
\begin{algorithm}[t!]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    %\underline{function Euclid} $(a,b)$\;
    %\Input{Initial iterate $w_0$}
	\While{not done}{
    Choose a batch of \textit{i.i.d.} tasks $\B_k \subseteq \I$ with distribution $p$ and with size $B = |\B_k|$;\\
    \For{all $\T_i$ with $i \in \B_k$}{
    Compute $\tilde{\nabla}f_i(w_k,\D_{in}^i)$  using dataset  $\D_{in}^i$;\\
    Set $w_{k+1}^i = w_k - \al \tilde{\nabla}f_i(w_k,\D_{in}^i)$;\\
    %Set $\tilde{\nabla}F_i(w_{k+1}^i)$ be an unbiased estimate of $\nabla F_i(w_{k+1}^i)$ using batches $\D_o^i, \D_h^i$;\\
    }
    Compute $w_{k+1}$ according to the update \eqref{hassan};
    \\
    $k \gets k + 1$;
    }
    \caption{\label{Algorithm1} MAML Algorithm}
\end{algorithm}

 In the inner step, for each task $\T_i$, we use a subset of the dataset $\D_{in}^i$ corresponding to task $\T_i$ to compute the stochastic gradient $\tilde{\nabla}f_i(w_k, \D_{in}^i)$ which is an an unbiased estimator of the gradient ${\nabla}f_i(w_k)$. The stochastic gradient $\tilde{\nabla}f_i(w_k, \D_{in}^i)$ is then used to compute a model $w_{k+1}^i$ corresponding to each task $\T_i$ by a single iteration of stochastic gradient descent, i.e.,
%%%
\begin{equation}\label{inner_step}
w_{k+1}^i = w_k - \al \tilde{\nabla}f_i(w_k,D_{in}^i).
\end{equation}
%%%%
To simplify the notation, we assume the size of dataset $\D_{in}^i$ for all tasks $i$ are equal to $D_{in}$.

In the outer loop, once we have the updated models $\{w_{k+1}^i\}_{i=1}^{B}$ for all tasks in $\B_k$, we compute the revised meta-model $w_{k+1}$ by performing the update 
%%%
%\begin{subequations} 
%\begin{align}
%& w_{k+1} = w_k - \be_k \frac{1}{B} \sum_{i \in \B_k}  \left(I-\al \tilde{\nabla}^2 f_i(w_{k},\D_{h}^i)\right)\ \! \tilde{\nabla} f_i\!\left(w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i\right) \label{hassan}\\
%&= w_k - \be_k \frac{1}{B} \sum_{i \in \B_k}  \left(I-\al \tilde{\nabla}^2 f_i(w_{k},\D_{h}^i)\right) \tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i) ,\label{hossein}
%\end{align}
%\end{subequations} 
%%%%
\begin{align}\label{hassan}
& w_{k+1} =  w_k - \be_k \frac{1}{B} \sum_{i \in \B_k}  \left(I-\al \tilde{\nabla}^2 f_i(w_{k},\D_{h}^i)\right) \tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i),
\end{align}
%%%%

where the stochastic gradient $\tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i) $ corresponding to task $\T_i$ is evaluated using the data set $\D_{o}^i$ and the models $\{w_{k+1}^i\}_{i=1}^{B}$ computed in the inner loop, and the stochastic Hessian $ \tilde{\nabla}^2 f_i(w_{k},\D_{h}^i)$ for each  task $\T_i$ is computed using the data set $\D_{h}^i$. Note that the data sets $\D_{in}^i$ used for the inner update are different from the data sets $\D_{o}^i$ and $\D_{h}^i$ used for the outer update. It is also possible to assume that $\D_{o}^i=\D_{h}^i$, but in this paper we assume that $\D_{o}^i$ and $\D_{h}^i$ are independent from each other that allows us to use a smaller batch for the stochastic Hessian computation which is more costly. Here also we assume that the sizes of $\D_o^i$ and $\D_h^i$ are fixed and equal to $D_o$ and $D_h$, respectively. The steps of MAML are outlined in Algorithm~\ref{Algorithm1}.




\vspace{2mm}
\noindent{\textbf{MAML as an approximation of SGD.}}
To better highlight the fact that MAML runs SGD over $F$ in \eqref{main_prob}, consider the update of GD for minimizing the objective function $F$ with step size $\beta_k$ which can be written as%\footnote{We are allowed to change the order of expectation and derivative as the number of tasks is finite.}
%%%
\begin{align}\label{GD_update}
& w_{k+1} = w_k - \be_k \nabla F(w_k) = w_k - \be_k \E_{i \sim p} \left [  \left(I-\al {\nabla}^2 f_i(w_{k})\right)\ \! {\nabla} f_i\!\left(w_k-\al {\nabla} f_i(w_k)\right) \right ] 
\end{align}
%%%
 As the underlying probability distribution of tasks $p$ is unknown, evaluation of the expectation in the right hand side of \eqref{GD_update} is often computationally prohibitive. Therefore, one can use SGD for minimizing the function $F$ with a batch $\B_k$ which contains $B$ tasks that are independently drawn. Then, the update is
 %%%
\begin{align}\label{SGD_update}
& w_{k+1} =  w_k - \frac{\be_k}{B} \sum_{i \in \B_k}  \left(I-\al {\nabla}^2 f_i(w_{k})\right)\ \! {\nabla} f_i\!\left(w_k-\al {\nabla} f_i(w_k)\right).
\end{align}
%%%

If we simply replace ${\nabla} f_i$ and ${\nabla}^2 f_i$ with their stochastic approximations over a batch of data points we obtain the update of MAML in~\eqref{hassan}.

%In the above update we have assumed that the exact gradients and Hessians of $f_i$, i.e., ${\nabla} f_i$ and ${\nabla}^2 f_i$, are available and we only sample the tasks. By comparing the updates in \eqref{hassan} and \eqref{SGD_update} we obtain that the update of MAML can be considered as a stochastic gradient descent on $F$ when we do not have access to the gradient ${\nabla} f_i$ and Hessian ${\nabla}^2 f_i$ of the loss associated with tasks and we approximate them by their stochastic variants. This is due to the fact that in many settings the function $f_i$ is defined either as the expectation over an infinite set of random functions or as the sum of a massive number of functions where each individual function is  associated with a sample of a very large dataset.


%Note that the gradient of the function $F(w)$ is given by
%\begin{subequations}\label{gradient_F}
%\begin{align}
%\nabla F(w) &= \sum_{i \in \I} p_i \nabla F_i(w), \label{gradient_F:a}\\
%\nabla F_i(w) &= A_i(w) \nabla f_i(w-\al \nabla f_i(w)) \label{gradient_F:b}
%\end{align}
%\end{subequations}
%with $A_i(w) := (I-\al \nabla^2 f_i(w))$. The update rule of SGD for solving problem \eqref{main_prob} is given by
%\begin{equation}\label{SGD_update}
%w_{k+1}^\text{SGD} = w_k^\text{SGD} - \beta \frac{1}{B} \sum_{i \in \B} p_i A_i(w_k^\text{SGD}) \nabla f_i(w_k^\text{SGD}-\al \nabla f_i(w_k^\text{SGD})) 
%\end{equation}
%where $\B$ is a sample batch of tasks with $B$ elements. In fact, if we approximate the matrix $A_i$ in \eqref{SGD_update} by the identity matrix, and also use sampling to estimate $\nabla f_i$, we will obtain Algorithm \ref{Algorithm1} from this update rule. As a result, MAML can be seen as an approximation of SGD.

%In what follows, we first show how Algorithm \ref{Algorithm1} can be interpreted as an approximation of Stochastic Gradient Descent (SGD) for minimizing the function $F$ in \eqref{main_prob} and then study its convergence using this novel interpretation. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{2mm}

\noindent{\textbf{Smaller batch selection for Hessian approximation.}} The use of first-order methods for solving problem~\eqref{main_prob} requires computing the gradient of $F$ which needs evaluating the Hessian of the loss $f_i$. Indeed, computation of the Hessians $\nabla^2 f_i$ for all the chosen tasks at each iteration is costly. % and is of order $\mathcal{O}(d^2B D_h )$, where $d$ is the dimension of the problem, $D_h$ is the size of batch used for stochastic Hessian approximation, and $B$ is the number of tasks chosen at each iteration for the update of MAML. 
One approach to lower this cost is to reduce the batch size $D_h$ used for Hessian approximation. Later in our analysis, we show that one can perform the update in \eqref{hassan} and have an exactly convergent method, while setting the batch size $D_h$ significantly smaller than batch sizes $D_{in}$ and $B$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t!]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    %\underline{function Euclid} $(a,b)$\;
    %\Input{Initial iterate $w_0$}
	\While{not done}{
    Choose a batch of \textit{i.i.d.} tasks $\B_k \subseteq \I$ with distribution $p$ and with size $B = |\B_k|$;\\
    \For{all $\T_i$ with $i \in \B_k$}{
    Compute $\tilde{\nabla}f_i(w_k,\D_{in}^i)$  using dataset  $\D_{in}^i$;\\
    Set $w_{k+1}^i = w_k - \al \tilde{\nabla}f_i(w_k,\D_{in}^i)$;\\
    %Set $\tilde{\nabla}F_i(w_{k+1}^i)$ be an unbiased estimate of $\nabla F_i(w_{k+1}^i)$ using batches $\D_o^i, \D_h^i$;\\
    }
    ${w_{k+1} \gets w_k -  ({\be_k}/{B}) \sum_{i \in \B_k}\tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i) }$; %using dataset $\D_{o}^i$
    \\
    $k \gets k + 1$;
    }
    \caption{\label{Algorithm2} First-Order MAML (FO-MAML)}
\end{algorithm}

\vspace{2mm}

\noindent{\textbf{First-order MAML (FO-MAML).}} To reduce the cost of implementing the update of MAML one might suggest ignoring the second-order term that appears in the update of MAML. In this approach, which is also known as first-order MAML (FO-MAML)  \citep{finn17a}, we update $w_k$ by following the update 
%%%%
\begin{equation}\label{FO_MAML}
w_{k+1} = w_k - \be_k \frac{1}{B} \sum_{i \in \B_k}  \tilde{\nabla} f_i(w_{k+1}^i ,\D_{o}^i),
\end{equation}
%%%
where the points $w_{k+1}^i$ are evaluated based on \eqref{inner_step}. Indeed, this approximation reduces the computational complexity of implementing MAML, but it comes at the cost of inducing an extra error in computation of the stochastic gradient of $F$. We formally characterize this error in our  theoretical results and show under what conditions the error induced by ignoring the second-order term does not impact its convergence. The steps of FO-MAML are outlined in Algorithm~\ref{Algorithm2}.






==> Final Draft/RelatedWorks.tex <==
%!TEX root = main.tex

\section{Related Work}\label{sec:RelatedWorks}

The problem of learning from prior experiences to learn new tasks efficiently has been formulated in various ways. One of the main approaches is designing algorithms for updating the parameters of the optimization methods used for training models \citep{bengio1990learning, bengio1992optimization}.
%This idea , where the authors studied the problem of learning how to update the parameters of a synaptic learning rule used for training neural networks. 
Recently, many papers have followed this approach \citep{bengio2012, NIPS2011_4443, li2016learning, ravi2016optimization} (see Table 1 in \citep{metz2018learning} for a summary of different approaches and also \citep{MetaLeatningSurvey} for a detailed survey). 
%including using random search for optimizing the hyper-parameters of the learner's model \citep{bengio2012, NIPS2011_4443}, learning the optimizer through the lens of reinforcement learning \citep{li2016learning}, or controlling the parameters of the gradient methods using recurrent neural networks \citep{ravi2016optimization} (see Table 1 in \citep{metz2018learning} for a summary of different approaches and also \citep{MetaLeatningSurvey} for a detailed survey). 
In one of the first theoretical formalizations, \cite{baxter2000model} 
%proposed a statistical framework with tasks drawn from a distribution, and 
study the problem of \textit{bias learning} where the goal is to find an automatic way for choosing the inductive bias in learning problems. Also, \cite{Franceschi_ICML18} provide a framework for tuning the hyper-parameters of learning algorithms, such as the initialization or the regularization parameter. %They investigate the asymptotic behavior of their method under additional assumptions, such as compactness of the hyper-parameter space and uniqueness of the optimal point for any choice of parameter.

In this paper, we focus on the theoretical analysis of gradient-based model-agnostic meta-learning methods. This setting was first introduced by \cite{finn17a}, and was followed {by several works proposing various algorithms \citep{Reptile, MAML++, Meta-SGD, CAVIA, alpha-MAML, grant2018recasting}. In particular,  \cite{grant2018recasting} introduce an adaptation of MAML for learning the parameters of a prior distribution in a hierarchical Bayesian model. \cite{Meta-SGD}, introduce a variant of MAML that replaces the inner loop learning rate with a vector (which is multiplied with the gradient in an element-wise manner) and then learns this step-vector as well. In another recent work, \cite{Reptile} introduce a new method named \textit{Reptile}, which samples a batch of tasks, and for each task, runs a few steps of stochastic gradient descent on its corresponding loss function. Reptile, then, takes the average from these resulting points and defines the next iterate to be the convex combination of this average and the current iterate.
 However, none of these works provide convergence guarantees for these MAML-type methods which is the main contribution of our paper.} 
\cite{finn19a} study MAML and its extension to online setting for strongly convex functions.
In a recent independent work, \cite{rajeswaran2019metalearning} propose iMAML which implements an approximation of one step of proximal point method in the inner loop. They show when the regularized inner loop loss function is strongly convex, iMAML converges to a first-order stationary point with exact gradient information (no stochasticity due to approximation by a batch of data) and under bounded gradient assumption. These assumptions remove the difficulties associated with unbounded smoothness parameter and biased gradient estimation featured in our analysis (Section~\ref{sec:Theory}).

The online version of meta learning
%, which is also related to the lifelong learning framework \citep{balcan2015efficient, pmlr-v54-alquier17a}, 
has also gained attention. In particular, \cite{balcan_ICML} consider the case where the agent sees a sequence of tasks, where each task is an online learning setup where the agent chooses its actions sequentially and suffer losses accordingly. For each task, the agent starts with an initial model, and runs a within task online algorithm to reduce the regret. Finally, the agent updates the initialization or regularization parameter using a meta-update online algorithm. The authors 
study this setting for convex functions and propose a framework using tools from online convex optimization literature. 
A closely related problem to this setting is the lifelong learning framework \citep{balcan2015efficient, pmlr-v54-alquier17a}. 
As an example, in \citep{pmlr-v54-alquier17a}, the authors consider the case were a series of tasks are presented sequentially where each task itself is associated with a dataset which is also revealed sequentially and processed by a within-task method. The authors focus on convex loss functions and introduce a meta-algorithm which updates a prior distribution on the set of feature maps, and use it to transfer information from the observed tasks to a new one.
In a similar line of work, \cite{Denevi_NeurIPS18,Denevi_ICML19} propose an algorithm which incrementally updates the bias regularization parameter using a sequence of observed tasks. 

Also, \cite{finn19a} consider the model-agnostic setting and propose follow the meta leader that achieves a sublinear regret.


==> Final Draft/acknowledgment.tex <==
%!TEX root = main.tex

\section{Acknowledgment}
Research was sponsored by the United States Air Force Research Laboratory and was accomplished under Cooperative Agreement Number FA8750-19-2-1000. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the United States Air Force or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation herein. Alireza Fallah acknowledges support from MathWorks Engineering Fellowship. The authors would like to thank Chelsea Finn and Zhanyu Wang for their comments on the first draft of this paper.


\vspace{6mm}


==> Final Draft/defs.tex <==
% latin-based symbols
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\la}{\lambda}
\newcommand{\de}{\delta}
\newcommand{\eps}{\epsilon}
\newcommand{\tsigma}{\tilde{\sigma}}

% linear algebra
\newcommand{\id}{I_d}
\newcommand{\zeros}{0_d}
\renewcommand{\vec}[1]
{\mbox{\boldmath${#1}$}}

% analysis
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\nn}{\nonumber}

%caligraphic 
\newcommand{\bigO}{\mathcal{O}}

% spaces
\newcommand{\R}{{\mathbb{R}}}

% operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\Tr}{Tr}

%optimization
\newcommand{\prox}{\text{prox}}

% paper-specific
\newcommand{\T}{\mathcal{T}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Sml}{$f\in S_{\mu,L}(\mathbb{R}^d)$ }

% environments
\newtheorem{theorem}{Theorem}[section]  % use one numbering scheme for all these objects
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conj}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}

% abbreviation for equations
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqs}{\begin{equation*}}
\newcommand{\eeqs}{\end{equation*}}
\newcommand{\beqas}{\begin{eqnarray*}}
\newcommand{\eeqas}{\end{eqnarray*}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% color boxes
\newtcbox{\mymath}[1][]{%
    nobeforeafter, math upper, tcbox raise base,
    enhanced, colframe=blue!30!black,
    colback=blue!30, boxrule=1pt,
    #1}
    
% comments
\def \ali#1{\textcolor{red}{#1}}
\def \alic#1{\textcolor{blue}{#1}}




==> Final Draft/theory.tex <==
%!TEX root = main.tex
\section{Theoretical Results}\label{sec:Theory}

In this section, we characterize the overall complexity of MAML, FO-MAML, and HF-MAML for finding a first-order stationary point of $F$ when the loss functions $f_i$ are nonconvex but smooth. 

\begin{definition}
A random vector $w_\eps\in \R^d$ is called an $\epsilon$-approximate first order stationary point (FOSP) for problem \eqref{main_prob} if it satisfies $
\E[ \Vert \nabla F(w_\eps) \Vert] \leq \eps$.
\end{definition}
%This definition implies that a point $w_\eps$ is an $\epsilon$-FOSP if its gradient norm for the global loss $F$ is smaller than $\epsilon$ in expectation. 


Our goal in this section is to answer two fundamental questions for each of the three considered methods. Can they find an $\epsilon$-FOSP for arbitrary $\eps>0$? If yes, how many iterations is needed for achieving such point? Before answering these questions, we first formally state our assumptions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%     A  S  S  U  M  P  T  I  O  N     %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{ass:boundedness}
$F$ is bounded below, $\min F(w)> -\infty$ and $\Delta\!:=\! (F(w_0) \!-\! \min_{w \in \R^d} F(w) )$ is bounded.
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%     A  S  S  U  M  P  T  I  O  N     %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{asm_smooth}
For every $i \in \I$, $f_i$ is twice continuously differentiable and $L_i$-smooth, i.e.,
\begin{equation*}
\Vert \nabla f_i(w) - \nabla f_i(u) \Vert \leq L_i \Vert w - u \Vert. 
\end{equation*}
\end{assumption}

%Since we also assume that the functions $f_i$ are twice differentiable, the $L_i$-smoothness assumption also implies that for every $w,u \in \R^d$ we have
%\begin{subequations} \label{smooth_2}
%\begin{align}
%&-L_i I_d \preceq \nabla^2 f_i(w) \preceq L_i I_d \quad \forall w \in \R^d,  \label{smooth_2:a}\\
%%- \frac{L_i}{2} \|w-u\|^2\leq  & \ 
%& f_i(w) - f_i(u) \!- \!\nabla f_i(u)^\top (w-u) \!\leq\! \frac{L_i}{2} \|w-u\|^2. \label{smooth_2:b}
%\end{align}
%\end{subequations}
For the simplicity of analysis, in the rest of the paper, we mostly work with $L:= \max_{i} L_i$ which can be considered as a parameter for the Lipschitz continuity of the gradients $\nabla f_i$ for all $i \in \I$.


%As we described in Section \ref{sec:MAML}, the Hessians $\nabla^2 f_i$ appear in the update of MAML. Hence, we need to impose a regularity condition on the variation of the Hessians expressed in the next Assumption, which is commonly used in the analysis of second-order methods.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%     A  S  S  U  M  P  T  I  O  N     %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{asm_Hesian_Lip}
For every $i \in \I$, the Hessian $\nabla^2 f_i$ is $\rho_i$-Lipschitz continuous, i.e., for every $w,u \in \R^d$, i.e., 
\begin{equation*}
\Vert \nabla^2 f_i(w) - \nabla^2 f_i(u) \Vert \leq \rho_i \Vert w - u \Vert.
\end{equation*}
\end{assumption}

To simplify our notation we use $\rho:=\max \rho_i$ as the Hessians Lipschitz continuity parameter for all $i \in \I$.
Note that we do not assume any smoothness conditions for the global loss $F$ and all the required conditions are for the individual loss functions $f_i$. In fact, later we show that under the conditions in Assumption~\ref{asm_smooth}, the global loss $F$ may not be gradient-Lipschitz in general.


The goal of Meta-learning is to train a model based on a set of given tasks so that this model can be used for learning a new unseen task. However, this is only possible if the training tasks are somehow related to unseen (test) tasks. In the following assumption, we formalize this condition by assuming that the gradient  $\nabla f_i$, which is an unbiased estimator of the gradient  $\nabla f= \E_{i \sim p}[\nabla f_i(w)]$, has a bounded variance. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%     A  S  S  U  M  P  T  I  O  N     %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{asm_bounded_var}
The variance of gradient $\nabla f_i(w)$ is bounded, i.e., for some $\sigma>0$ we have
\begin{equation}\label{bounded_var}
 \E_{i \sim p}[\| \nabla f(w) - \nabla f_i(w)\|^2] \leq \sigma^2.
\end{equation}
\end{assumption}

{Note that this assumption is less strict comparing to the bounded gradient assumption in \citep{finn19a, rajeswaran2019metalearning}. In addition, for strongly convex functions, this assumption is closely related to the one in \citep{balcan_ICML} which states the optimal point of loss functions of all tasks are within a ball where its radius quantifies the similarity.}
%The condition in Assumption~\ref{asm_bounded_var} shows that each individual stochastic gradient $\nabla f_i(w)$ is an unbiased estimator of the expected gradient $\nabla f(w):= \E_{i \sim p}[\nabla f_i(w)]$ with a bounded variance, and these conditions are customary in stochastic optimization. 

%As we stated in the introduction, in many applications, evaluating the exact gradient corresponding to the loss function of each task is computationally costly, and we only have access to a batch of data to compute an unbiased estimator of the exact gradient $\nabla f_i(w)$. %For instance, if the loss function $f_i$ for each task $\T_i$ is defined as the expectation of a set of random functions $f_i(w) = \E_\theta [f_i(w, \theta)] $ where $\theta$ is a random variable or defined as the average of a large number of functions $f_i(w) = \frac{1}{|\D|} \sum_{j\in \D} [f_i(w, \theta_j)]$. 
In the following assumption we formally state the conditions required for the stochastic approximations of the gradients $\nabla f_i(w, \theta)$ and Hessians $\nabla^2 f_i(w, \theta)$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%     A  S  S  U  M  P  T  I  O  N     %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{asm_bounded_var_i}
For any $i$ and any $w\in \R^d$, the stochastic gradients $\nabla f_i(w, \theta)$ and Hessians $\nabla^2 f_i(w, \theta)$ have bounded variance, i.e., 
\begin{align}
&\E_\theta[\| \nabla f_i(w, \theta) - \nabla f_i(w)\|^2] \leq \tilde{\sigma}^2, \label{bounded_var_i} \\
&\E_\theta[\| \nabla^2 f_i(w, \theta) - \nabla^2 f_i(w)\|^2] \leq \sigma_H^2, \label{bounded_hess_i}  
\end{align}

where $\tsigma$ and $\sigma_H$ are non-negative constants.
\end{assumption}

%In particular, it is worth noting that the special case $\tsigma=\sigma_H=0$ represents the case that the exact gradient and Hessian for each task is available.  %In our theoretical results we consider the general case $\tsigma>0, \sigma_H> 0$ and the special case $\tsigma=\sigma_H=0$.

Finally, to simplify the statement of our results for MAML, FO-MAML, and HF-MAML, we make the following assumption on the relation of parameters. {Later in the appendix, we drop this assumption and state the \textit{general version} of our results.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%     A  S  S  U  M  P  T  I  O  N     %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{asm_simplify}
%Recall the definitions $L:=\max L_i$ and $\rho:=\max \rho_i$ with $L_i$ and $\rho_i$ defined in Assumptions \ref{asm_smooth} and \ref{asm_Hesian_Lip}, respectively. Then, 
We assume $\rho \alpha/L = \bigO(1)$. Also, we assume $\sigma^2 + \tsigma^2 = \bigO(1)$, where $\sigma$ and $\tsigma$ are defined in Assumptions \ref{asm_bounded_var} and \ref{asm_bounded_var_i}, respectively.
\end{assumption}

%\begin{remark}
%We would like to emphasize that all the conditions in Assumption~\ref{asm_simplify} are added only to simplify the statements of our main theorems. All our results hold even if Assumption~\ref{asm_simplify} is not satisfied. In fact, in the appendix, we state our proofs for the general case in which Assumption~\ref{asm_simplify} does not hold.  
%\end{remark}


\subsection{Challenges in analyzing MAML methods}\label{AnalysisChallenges}


Before stating our main results for MAML, FO-MAML, and HF-MAML, in this subsection we briefly highlight some of the challenges that emerge in analyzing these algorithms and prove some intermediate lemmas that we will use in the following subsections. 

\noindent{\textbf{(I) Unbounded smoothness parameter:}} %As we mentioned in the previous section,
The global loss function $F$ that we are minimizing in the MAML algorithm by following a stochastic gradient descent step is not necessarily smooth over $\R^d$, and its smoothness parameter could be unbounded. We formally characterize the parameter for the Lipschitz continuity of the gradients $\nabla F$ in the following lemma.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        L  E  M  M  A       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem_smooth_F}
Consider the objective function $F$ defined in \eqref{main_prob} for the case that $\al \in [0, \frac{1}{L}]$. Suppose that the conditions in Assumptions~\ref{asm_smooth}-\ref{asm_Hesian_Lip} are satisfied. 
%, and recall the definitions $L:=\max L_i$ and $\rho:=\max \rho_i$. 
Then, for any $w,u \in \R^d$ we have
\begin{align}\label{smooth_F}
& \Vert \nabla F(w) - \nabla F(u) \Vert \leq \min \{ L(w), L(u)\} \Vert w \!-\! u \Vert.
%& \left(4L \!+\! 2 \rho \al \min\{\E_{i \sim p} \|\nabla f_i(w)\|,\E_{i \sim p} \|\nabla f_i(u)\|\}\right) \Vert w \!-\! u \Vert. \nonumber   
\end{align}
where $L(w) := 4L \!+\! 2 \rho \al \E_{i \sim p} \|\nabla f_i(w)\|$.
\end{lemma}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        P  R  O  O  F       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{proof}
%Check Appendix \ref{lem_smooth_F_proof}.
%\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
The result in Lemma~\ref{lem_smooth_F} shows that the objective function $F$ is smooth with a parameter that depends on the minimum of the expected norm of gradients. In other words, when we measure the smoothness of gradients between two points $w$ and $u$, the smoothness parameter depends on $\min\{\E_{i \sim p} \|\nabla f_i(w)\|,\E_{i \sim p} \|\nabla f_i(u)\|\}$. Indeed, this term could be unbounded or arbitrarily large as we have no assumption on the gradients norm. Moreover, computation of $\min\{\E_{i \sim p} \|\nabla f_i(w)\|,\E_{i \sim p} \|\nabla f_i(u)\|\}$ could be costly as it requires access to the gradients of all tasks.

% Before moving to next challenge in analyzing MAML, we use Lemma~\ref{lem_smooth_F} to show the following result.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%        C  O  R  O  L  L  A  R  Y         %%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{corollary}\label{bergman_bound}
%Let $\al \in [0, \frac{1}{L}]$. Then, for  $w,u \in \R^d$,
%
%\begin{equation}
%F(u) - F(w) - \nabla{F}(w)^\top (u-w) \leq \frac{L(w)}{2} \|u-w \|^2,
%\end{equation}
%where $L(w)  = 4L + 2 \rho \al \E_{i \sim p} \|\nabla f_i(w)\|$. 
%\end{corollary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent{\textbf{(II) Stochastic stepsize:}} For most optimization methods, including SGD, the stepsize is selected proportional to the inverse of the smoothness parameter. However, in our setting, this parameter depends on the norm of gradient of all tasks which is not computationally tractable. To resolve this issue, we propose a method for choosing the stepsize $\beta_k$ by approximating $L(w)$ with an average over a batch of tasks. Specifically, we approximate $\E_{i \sim p} \|\nabla f_i(w)\|$ in the definition of $L(w)$ using the estimator $\sum_{j \in \B'} \|\tilde{\nabla} f_j(w, \D_\beta^j)\|$ where $\D_\beta^j$ is a dataset corresponding to task $j$ with size $D_\beta$. Hence, we estimate $L(w)$ by
%%

\begin{equation}\label{el_tilde_def}
\tilde{L}(w):={4L + \frac{2\rho \al}{B'} \sum_{j \in \B'} \|\tilde{\nabla} f_j(w, \D_\beta^j)\|  }.
\end{equation} 
%%%
Using this estimate, our stepsize $\beta_k$ is tuned to be a constant times the inverse of $\tilde{L}(w)$ which we denote by  $\tilde{\be}(w)=1/\tilde{L}(w)$, i.e., $\beta_k=c\tilde{\be}(w)=c/\tilde{L}(w)$. This simple observation shows that the stepsize that we need to use for MAML algorithms is stochastic as $1/\tilde{L}(w)$ is a random parameter and depends on the choice of $\B'$. Therefore, we need to derive lower and upper bounds on the  expectations $E[\beta_k]$ and $\E[\beta_k^2]$, respectively, as they appear in the convergence analysis of gradient-based methods. Considering the defintion $\beta_k=c\tilde{\be}(w)$, we state these bounds for $\tilde{\be}(w)$ in the following lemma.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        L  E  M  M  A       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{tilde_beta}
Consider the function $F$ defined in \eqref{main_prob} for the case that $\al \in [0, \frac{1}{L}]$. Suppose Assumptions~\ref{asm_smooth}-\ref{asm_bounded_var_i} hold.
%, and recall the definitions $L:=\max L_i$ and $\rho:=\max \rho_i$. 
Further, consider the definition 
%%%

\begin{equation}\label{beta_update}
\tilde{\be}(w) \! :=\! \frac{1}{\tilde{L}(w)}\!:=\! \frac{1}{4L\! +\! 2 \rho \al \sum_{j \in \B'} \|\tilde{\nabla} f_j(w, \D_\beta^j)\| /{B'} },
\end{equation}
where $\B'$ is a batch of tasks with size $B'$ which are independently drawn with distribution $p$, and for every $j \in \B'$, $\D_\beta^j$ is a dataset corresponding to task $j$ with size $D_\beta$. If the conditions 
%%%%

\begin{equation}\label{size_B'}
B' \geq \ceil[\big]{0.5 \left({\rho \al \sigma}/{L}\right)^2}, \quad D_\beta \geq \ceil[\big]{\left({2 \rho \al \tsigma}/{L}\right)^2}
\end{equation}
%%%%
are satisfied, then we have

\begin{equation} \label{first_second_moment}
\E \left[\tilde{\be}(w)\right] \geq  \frac{0.8}{L(w)}, \quad \E\left[\tilde{\be}(w)^2\right] \leq \frac{3.125}{L(w)^2}
\end{equation}
where $L(w)= 4L + 2 \rho \al \E_{i \sim p} \|\nabla f_i(w)\|$.
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        P  R  O  O  F       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{proof}
%Check Appendix \ref{tilde_beta_proof}.
%\end{proof}    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Lemma \ref{tilde_beta} shows that if we set
%the parameter $\beta(w_k)$ in the expression for 
 $\beta_k=c\tilde{\beta}(w_k)$, with $\tilde{\beta}(w_k)$ given
%based on the expression 
in \eqref{beta_update} and the batch-sizes $B'$ and $D_\beta$ satisfy the conditions \eqref{size_B'}, then the first moment of  $\beta_k$ is bounded below by a factor of $1/L(w_k)$ and its second moment is upper bounded by a factor of $1/L(w_k)^2$. 

Throughout the paper, we assume at each iteration $k$, the batches $\B'_k, \{\D_\beta^j\}_{j \in \B'_k}$ are independently drawn from $\B_k$ and $\{\D_{in}^i, \D_o^i, \D_h^i\}_{i \in \B_k}$ used in the updates of MAML methods.
Also, it is worth emphasizing that the batch size for the random sets $\B'_k$ and $ \{\D_\beta^j\}_{j \in \B'_k}$ are independent of the desired accuracy $\epsilon$ and the extra cost for the computation of these batches is of $\mathcal{O}(1)$. 


\noindent{\textbf{(III) Biased estimator:}} The statement that MAML performs an update of stochastic gradient descent at each iteration on the objective function $F$ is not quite accurate. To better highlight this point, recall the update of MAML in \eqref{hassan}. According to this update, the descent direction $g_k$ for MAML at step $k$ is given by
%%%

\begin{equation*}
g_k:= \frac{1}{B} \sum_{i \in \B_k}  A_{i,k}\ \! \tilde{\nabla} f_i\!\left(w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i\right),
\end{equation*} 
%%%
with $A_{i,k}:=(I-\al \tilde{\nabla}^2 f_i(w_{k},D_{h}^i))$, while the exact gradient of $F$ at $w_k$ is given by 
%%%
\begin{equation*}
\nabla F(w_k)\!= \!\E_{i \sim p} \left [\! \left(I\!-\!\alpha \nabla^2 f_i(w_k)\right)  \!\nabla f_i(w_k\!-\!\al \nabla f_i(w_k))\! \right ]\!.
\end{equation*} 
%%%
Given $w_k$, $g_k$ is not an unbiased estimator of the gradient $\nabla F(w_k)$ as the stochastic gradient $\tilde{\nabla} f_i(w_k,\D_{in}^i)$ is within the stochastic gradient $\tilde{\nabla} f_i (w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i)$. Hence, the descent direction that we use in the update of MAML for updating models is a biased estimator of $\nabla F(w_k)$. This is another challenge that we face in analyzing MAML and its variants. To overcome this challenge, we need to characterize the first-order and second-order moments of the expression $\tilde{\nabla} f_i (w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i)$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        L  E  M  M  A       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lemma:moments}
Consider $F$ in \eqref{main_prob} for the case that $\al \in [0, \frac{1}{L}]$. Suppose Assumptions~\ref{asm_smooth}-\ref{asm_bounded_var_i} hold.
%, and recall the definitions $L:=\max L_i$ and $\rho:=\max \rho_i$. 
Then, 
%%%

\begin{align}\label{bias}
&\E_{\D_{in},\D_o}[\tilde{\nabla} f_i (w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i) \mid \F_k]= \nabla f_{i} \left  (w_k \!-\! \alpha \nabla f_{i}(w_k) \right ) +e_{i,k} ,\  \text{where} \   \|e_{i,k} \| \leq \frac{\al L\tsigma}{\sqrt{D_{in}}}.
\end{align}
%%%
Moreover, for arbitrary $\phi>0$ we have
%%%
\begin{align}\label{sec_moment}
 \E_{\D_{in},\D_o} \!\left [ \|\tilde{\nabla} f_i (w_k\!-\!\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i)\|^2  \mid \F_k \right]  \leq & \left(1+\frac{1}{\phi}\right)\|\nabla f_{i} (w_k - \alpha \nabla f_{i}(w_k))\|^2\nonumber\\
  & +  \frac{(1\!+\!\phi) \al^2 L^2\tsigma^2}{D_{in}}+ \frac{\tsigma^2}{D_o}.
\end{align}
%%% 
\end{lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        P  R  O  O  F       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{proof}
%Check Appendix \ref{lemma:moments_proof}.
%\end{proof}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The result in Lemma~\ref{lemma:moments} clarifies the reason that the descent direction of MAML denoted by $g_k$ is a biased estimator of $\nabla F(w_k)$. It shows that the bias is bounded above by a constant which depends on the variance of the stochastic gradients $\tilde{\nabla} f_i$ and the stepsize $\alpha$ for the inner steps. By setting $\alpha=0$, the vector $\tilde{\nabla} f_i (w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i)$ becomes an unbiased estimate of $\nabla f_{i} (w_k - \alpha \nabla f_{i}(w_k) )$ as our result in \eqref{bias} also suggests. Also, the result in \eqref{sec_moment} shows that the second moment of $\tilde{\nabla} f_i (w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i)$ is bounded above by the sum of a multiplicand of  $\|\nabla f_{i} (w_k - \alpha \nabla f_{i}(w_k) )\|^2$ and a multiplicand of $\tilde{\sigma}^2$. %For the special case of $\alpha=0$, we would expect the second moment of $\tilde{\nabla} f_i (w_k-\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i)$ to be bounded above by $\|\nabla f_{i} (w_k - \alpha \nabla f_{i}(w_k) )\|^2+\tilde{\sigma}^2/D_o$, which can also be obtained from \eqref{sec_moment} by setting $\phi \to \infty$.


%\begin{align}
%\nabla F(w) &= \sum_{i \in \I} p_i \nabla F_i(w), \label{gradient_F:a}\\
%\nabla F_i(w) &= A_i(w) \nabla f_i(w-\al \nabla f_i(w)) \label{gradient_F:b}
%\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{On the Connection of $F$ and $\hat{F}$}




In this subsection, we investigate the connection between $F$ and $\hat{F}$ defined in \eqref{main_prob} and \eqref{main_prob_2}, respectively. In particular, in the following theorem, we characterize the difference between their gradients. Later, using this result, we show all the methods that we study achieve the same level of gradient norm with respect to both $F$ and $\hat{F}$, up to some constant.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        THEOREM       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{Thm_F_hatF}
Consider the functions $F$ and $\hat{F}$ defined in \eqref{main_prob} and \eqref{main_prob_2}, respectively, for the case that $\al \in (0,\frac{1}{L}]$. Suppose Assumptions~\ref{asm_smooth}-\ref{asm_bounded_var_i} hold.
%, and recall the definitions $L:=\max L_i$ and $\rho:=\max \rho_i$. 
Then, for any $w \in \R^d$, we have

\begin{equation}
\|\nabla \hat{F}(w) - \nabla F(w)\| \leq 2 \alpha L \frac{\tsigma}{\sqrt{D_{test}}} + \alpha^2 L \frac{\sigma_H \tilde{\sigma}}{D_{test}}.	
\end{equation}
\end{theorem}
%\begin{proof}
%Check Appendix \ref{proof_Thm_F_hatF}.	
%\end{proof}
Next, we mainly focus on characterizing the behavior of MAML, FO-MAML, and HF-MAML with respect to $F$, and by using the above theorem, we can immediately obtain bounds on the norm of $\nabla \hat{F}$ as well. In fact, the above theorem indicates the difference between $\nabla F$ and $\nabla \hat{F}$ is $\bigO (\max\{\frac{\tsigma}{\sqrt{D_{test}}}, \frac{\sigma_H \tilde{\sigma}}{D_{test}}\} )$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Convergence of MAML}



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{theorem}\label{Thm_GD_det}
Consider running GD with update rule \eqref{SGD_update} and $\B = \I$. Let $\al \in (0,\frac{1}{4L}]$ and $\beta_k =\frac{1}{L_k}$ with
\begin{equation}\label{L_k}
L_k  = 4L + 2 \rho \al \E_{i \sim p} \|\nabla f_i(x_k)\|.    
\end{equation}
Also, assume that we have access to the exact gradients in all steps, i.e., $\tilde{\nabla} f_i(x) = \nabla{f_i}(x)$. Then GD finds an $\eps$-approximate first order stationary solution for problem \eqref{main_prob} after at most 
\begin{equation*}
\Delta \max \left \{ \frac{16L + 24 \rho \al \sigma }{\eps^2}, \frac{24 \rho \al}{\eps}   \right \}    
\end{equation*}
iterations where $\Delta$ is the optimality gap, i.e., $\Delta = F(x_0) - \min_{x \in \R^d} F(x)$.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Corollary \ref{bergman_bound} implies
\begin{align}
F(x_{k+1}) & \leq  F(x_k) + \nabla{F}(x_k)^\top (x_{k+1}-x_k) + \frac{L_k}{2} \| x_{k+1}-x_k \|^2  \\
& =  F(x_k) - \be_k \| \nabla{F}(x_k)\|^2 + \frac{L_k}{2} \be_k^2 \| \nabla{F}(x_k)\|^2 \label{thm1_eq1}\\
& =  F(x_k) - \frac{1}{2L_k} \| \nabla{F}(x_k)\|^2 \label{thm1_eq2}
\end{align}
where \eqref{thm1_eq1} follows from the GD update rule and \eqref{thm1_eq2} is obtained by substituting $\be_k$ by its upper bound $\frac{1}{L_k}$. As a result, at iteration $k$, the decrease in function value is at least $\frac{1}{2L_k} \| \nabla{F}(x_k)\|^2$. This amount can be lower bounded as follows
\begin{align}
\frac{1}{2L_k} \| \nabla{F}(x_k)\|^2 &= \frac{\| \nabla{F}(x_k)\|^2}{2(4L + 2 \rho \al \E_{i \sim p} \|\nabla f_i(x_k)\|)}  \\
& \geq \frac{\| \nabla{F}(x_k)\|^2}{2(4L + 2 \rho \al \sigma + 2 \rho \al \|\nabla f(x_k)\|)} \label{thm1_ineq1}
\end{align}
where the last inequality follows from \eqref{lem2_ineq4}. Using Lemma \ref{lemma_bound_by_F} along with the fact that $\al \leq \frac{1}{4L}$, implies
\begin{equation}\label{thm1_ineq2}
\|\nabla f(x_k)\| \leq 3 \| \nabla{F}(x_k)\| + 2 \sigma.
\end{equation}
Plugging \eqref{thm1_ineq2} in \eqref{thm1_ineq1} yields
\begin{align}
\frac{1}{2L_k} \| \nabla{F}(x_k)\|^2 & \geq \frac{\| \nabla{F}(x_k)\|^2}{8L + 12 \rho \al \sigma + 12 \rho \al \| \nabla{F}(x_k)\|} \\
& \geq \frac{\| \nabla{F}(x_k)\|^2}{2 \max \{ 8L + 12 \rho \al \sigma, 12 \rho \al \| \nabla{F}(x_k)\| \} }  \\
& = \min \left \{  \frac{\| \nabla{F}(x_k)\|^2}{16L + 24 \rho \al \sigma }, \frac{\| \nabla{F}(x_k)\|}{24 \rho \al}   \right \} \label{thm1_ineq3}. 
\end{align}
Therefore, by using \eqref{thm1_ineq3} in \eqref{thm1_ineq1}, we obtain 
\begin{align*}
F(x_{k+1}) & \leq  F(x_k) - \min \left \{  \frac{\| \nabla{F}(x_k)\|^2}{16L + 24 \rho \al \sigma }, \frac{\| \nabla{F}(x_k)\|}{24 \rho \al}   \right \}.
\end{align*}
Hence, at iteration $k$, if $\| \nabla{F}(x_k)\| \geq \eps$, the amount of function value decrease will be at least 
\begin{equation*}
\min \left \{  \frac{\eps^2}{16L + 24 \rho \al \sigma }, \frac{\eps}{24 \rho \al}   \right \}
\end{equation*}
which gives the given rate in the theorem statement.
\end{proof}
Using this result, we next state the convergence of SGD for Problem \eqref{main_prob}.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this subsection, we study the overall complexity of MAML for finding an $\eps$-FOSP of the loss functions $F$ and $\hat{F}$ defined in \eqref{main_prob} and \eqref{main_prob_2}, respectively.  
%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        THEOREM       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{Thm_SGD_general_simple} 
Consider $F$ in \eqref{main_prob} for the case that $\al \in (0,\frac{1}{6L}]$. Suppose Assumptions~\ref{ass:boundedness}-\ref{asm_simplify} hold.
%, and recall the definitions $L:=\max L_i$ and $\rho:=\max \rho_i$. 
Consider running MAML with batch sizes satisfying the conditions $D_h \geq \ceil{2 \al^2 \sigma_H^2}$ and $B \geq 20$.
Let $\beta_k = \tilde{\beta}(w_k)/12$
where $\tilde{\beta}(w)$ is given in \eqref{beta_update}.
Then, for any $1>\eps >0$, MAML finds a solution $w_\eps$ such that
%%%%

\begin{equation}
 \E[ \| \nabla F(w_\eps) \|] \leq \bigO \left ( \sqrt{\frac{\sigma^2}{B} + \frac{\tsigma^2}{B D_o} + \frac{\tsigma^2}{D_{in}}} \right ) + \eps	
\end{equation}
with a total number of iterations of

\begin{equation}
\bigO(1) \Delta \min \left \{ \frac{L}{\eps^2},
\frac{LB}{\sigma^2} + \frac{L(B D_o+D_{in})}{\tsigma^2} \right \} .
\end{equation}
\end{theorem}
%%%%%%%%%%% Proof %%%%%%%%%%%%
%\begin{proof}
%Check Appendix \ref{Thm_SGD_general_proof} for the general statement of the theorem and its proof.
%\end{proof}
%\begin{remark}
%It is worth noting that the condition $B \geq 20$ can be dropped, i.e., $B$ can be any positive integer, at the cost of 	decreasing the ratio $\beta_k / \tilde{\beta}(w_k)$.
%\end{remark}
The result in Theorem~\ref{Thm_SGD_general_simple}  shows that after running MAML for $\mathcal{O}(\frac{1}{\eps^2}+ \frac{B}{\sigma^2} + \frac{BD_o+D_{in}}{\tsigma^2})$ iterations, we can find a point $w^{\dag}$ that its expected gradient norm  $\E[ \| \nabla F(w^{\dag}) \|] $ is at most of $\eps+ \mathcal{O}( \sqrt{ \frac{\sigma^2}{B} +\frac{ \tsigma^2}{B D_o} + \frac{ \tsigma^2}{D_{in}}})$. This result implies that if we choose the batch sizes $B$, $D_o$, and $D_{in}$ properly (as a function of $\eps$), then for any $\eps>0$ it is possible to reach an $\eps$-FOSP of problem \eqref{main_prob} in a number of iterations which is polynomial in $1/\eps$. We formally state this result in the following corollary.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%       COROLLARY       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}\label{cor_large_batch_MAML}
Suppose the condition in Theorem~\ref{Thm_SGD_general_simple} are satisfied. Then, if the batch sizes $B$, $D_o$, and $D_{in}$ satisfy the following conditions, 
%%%

\begin{equation}
B \geq  (C_1 {\sigma^2})/{\eps^2}, \quad D_{in}, BD_o \geq (C_2 {\tsigma^2})/{\eps^2},
\end{equation}
for some constants $C_1$ and $C_2$, then MAML finds an $\eps$-FOSP after $\Delta \bigO ({L}/{\eps^2})$ iterations.
\end{corollary}


The result shows that with sufficient samples for the batch of stochastic gradient evaluations, i.e.,  $D_{in}$ and $D_{o}$, and for the batch of tasks $B$, MAML finds an $\eps$-FOSP after at most $\mathcal{O}(1/\eps^2)$ iterations for any $\eps>0$. 
\begin{comment}
In the next corollary, we characterize the complexity of MAML for the special case that exact gradients and hessian are available for each task, i.e., $\tsigma=\sigma_H=0$, and only tasks are randomly chosen.  

\begin{corollary}\label{cor_MAML_det}
Suppose the condition in Theorem~\ref{Thm_SGD_general} are satisfied. Further, assume that 
we have access the exact values of $\nabla f_i$ and $\nabla^2 f_i$ in inner and outer loops.
Then, for any $\eps >0$, MAML with batch size
\begin{equation}
B \geq \max \left \{20, \frac{56 \sigma^2(L + \rho \alpha \sigma)}{L \eps^2} , \frac{28 \rho \alpha \sigma^2}{L\eps} \right \}    
\end{equation}
finds an $\eps$-FOSP point, i.e., $\E[\|\nabla F(w)\|]\leq \eps$, in at most 
$\bigO(1) \Delta (L + \rho \al (\sigma + \eps))/{\eps^2}$
iterations, where $\Delta:= (F(w_0) - \min_{w \in \R^d} F(w) )$.
\end{corollary} 
\end{comment}
%%%%%%%%%%%%%%%%%% Remark %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{remark}
\sloppy Based on Theorem \ref{Thm_F_hatF}, the difference between $\nabla F$ and $\nabla \hat{F}$ is $\bigO \left (\max\{\frac{\tsigma}{\sqrt{D_{test}}}, \frac{\sigma_H \tilde{\sigma}}{D_{test}}\} \right )$. Given that, and since in practice, we usually choose $D_{test}$ at least as large as $D_{in}$, one can see that as long as $\sigma_H$ is not significantly larger than $\tilde{\sigma}$, the order of norm of gradient for both $F$ and $\hat{F}$ would be similar for all the results, up to some constant. This argument holds for FO-MAML and HF-MAML as well. 	
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}
%\begin{theorem}\label{Thm_SGD}
%Consider running MAML with having access to the exact values of $\nabla f_i$ and $\nabla^2 f_i$ in inner and outer loops.
%%with update rule 
%%\begin{equation}
%%w_{k+1} = w_k - \beta_k \frac{1}{|\B_k|} \sum_{i \in \B_k} \nabla{F}_i(w_k) 
%%\end{equation}
%%where each task in batch $\B_k$ is chosen independently from others with distribution $p$. 
%Let $\al \in (0,\frac{1}{4L}]$ and $\beta_k = \tilde{\beta}(w_k)/3$
%where $\tilde{\beta}(w)$ is given in Lemma \ref{tilde_beta} and is computed over a batch $\B'_k$ independently drawn from $\B_k$.
%%Also, assume that we have access to the exact gradients in all steps, i.e., $\tilde{\nabla} f_i(w) = \nabla{f_i}(w)$. 
%Then, for any $\eps >0$, MAML with batch size
%\begin{equation*}
%B \geq \max \left \{16, \frac{(36L + 54 \rho \al \sigma) \sigma^2 }{\eps^2 L} , \frac{54 \rho \al \sigma^2}{\eps L}   \right \}    
%\end{equation*}
%finds a solution $w_\eps$ such that
%\begin{equation}
% \E[ \| \nabla F(w_\eps) \|] \leq \eps
%\end{equation}
%after at most
%\begin{equation*}
%%N_\eps^{\text{MAML}} :=72 \Delta \max \left \{ \frac{2L + 3 \rho \al \sigma }{\eps^2}, \frac{3 \rho \al}{\eps}   \right \} 
%\bigO(1) \Delta \max \left \{ \frac{L + \rho \al \sigma }{\eps^2}, \frac{\rho \al}{\eps}   \right \} 
%\end{equation*}
%iterations.
%\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\subsubsection{Convergence of K-shot MAML}
%%The next theorem characterize the convergence of MAML when the gradients of inner loop and outer loop are computed using batches (see Appendix \ref{Thm_SGD_general_proof} for the proof).
%with update rule 
%\begin{equation}
%w_{k+1} = w_k - \beta_k \frac{1}{B} \sum_{i \in \B_k} \tilde{\nabla{F}_i}(w_k) 
%\end{equation}
%where each task in batch $\B_k$ is chosen independently from others with distribution $p$. In addition, $\tilde{\nabla{F}_i}(w_k)$ is given by
%\begin{equation}
%\tilde{\nabla{F}_i}(w_k) = \left (I - \al \frac{1}{\D_h} \sum_{j \in \D_h^i} \nabla^2 f_{i,j}(w_k)\right ) \left ( \frac{1}{\D_o} \sum_{p \in \D_o^i} \nabla f_{i,p}\left (w_k - \alpha \frac{1}{\D_{in}} \sum_{q \in \D_{in}^i} \nabla f_{i,q}(w_k)\right ) \right )     
%\end{equation}
%where $\D_{in}^i, \D_o^i,$ and $\D_h^i$ are three batches drawn independently from $S_i$, with size $D_{in}, D_o,$ and $D_h$, respectively.	
%\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{remark}
%The assumption $B \geq 20$ in both results can be relaxed by decreasing the stepsize to $\beta_k = \tilde{\beta}(w_k)/100$. 	
%\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Convergence of FO-MAML}




Now we proceed to characterize the convergence of the first order approximation of MAML (FO-MAML). %presented in Algorithm~\ref{Algorithm2}. %In particular, we first characterize the overall complexity of this algortihm for finding a first-order stationary point of the function $F$. 
%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%        THEOREM       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}\label{First_order_MAML_det_simple}
Consider $F$ in \eqref{main_prob} for the case that $\al \in (0,\frac{1}{10L}]$. Suppose Assumptions~\ref{ass:boundedness}-\ref{asm_simplify} hold. %, and recall the definitions $L:=\max L_i$ and $\rho:=\max \rho_i$. 
Consider running FO-MAML with batch sizes satisfying the conditions $D_h \geq \ceil{2 \al^2 \sigma_H^2}$ and $B \geq 20$.
Let $\beta_k = \tilde{\beta}(w_k)/18$
where $\tilde{\beta}(w)$ is defined in \eqref{beta_update}.
Then, for any $1>\eps >0$, FO-MAML finds $w_\eps$ such that
%%%%
\begin{equation}\label{result_FOMAML_general_simple}
\E  [ \| \nabla F(w_\eps) \|] \!\leq \!\bigO\! \left (\! \sqrt{\sigma^2\! \left( \!\alpha^2 L^2\!+\!\frac{1}{B}\!\right)\! +\! \frac{\tsigma^2}{B D_o} \!+\! \frac{\tsigma^2}{D_{in}}} \right )\!	+\! \eps
\end{equation}
with a total number of iterations of

\begin{equation*}
\bigO(1) \Delta \min \left \{ \frac{L}{\eps^2}, \frac{L}{\sigma^2 (\alpha^2 L^2\!+\!{B^{-1}})}+\frac{L(BD_o\!+\!D_{in})}{\tsigma^2} \right \}\!.
\end{equation*}
%iterations, where $\Delta:= (F(w_0) - \min_{w \in \R^d} F(w) )$.
\end{theorem}
%\begin{proof}
%Check Appendix \ref{First_order_MAML_det_proof} for the general statement of the theorem and its proof.
%\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Comparing Theorem~\ref{First_order_MAML_det_simple} with Theorem \ref{Thm_SGD_general_simple} implies that FO-MAML, in contrast to MAML, may not converge to an exact first-order stationary point even when we use large batch sizes (see the subsection below). Specifically, even if we choose large batch sizes $B$, $D_{in}$, and $D_o$ for FO-MAML, the  gradient norm cannot become smaller than $\mathcal{O}(\alpha \sigma)$. This is because of the $\alpha^2 L^2 \sigma^2$ term in \eqref{result_FOMAML_general_simple} which does not decrease by increasing the batch sizes for the tasks and stochastic gradient evaluations.
Now we state the results for FO-MAML when, as in corollary \ref{cor_large_batch_MAML}, we use batch sizes of $\mathcal{O}(1/\eps^2)$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%       COROLLARY       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}
Suppose the condition in Theorem~\ref{First_order_MAML_det_simple} are satisfied. Then, if the batch sizes $B$, $D_o$, and $D_{in}$ satisfy the following conditions, 
%%%
\begin{comment}

\begin{equation}
D_{in}\geq \frac{8\tsigma^2}{L} \left(\frac{L + \rho \al (\sigma + \eps) }{\eps^2} \right),
\ 
B \geq \frac{35\sigma^2}{L} \left(\frac{L + \rho \al (\sigma + \eps) }{\eps^2} \right),
\ 
BD_o \geq \frac{5\tsigma^2}{L} \left(\frac{L + \rho \al (\sigma + \eps) }{\eps^2} \right),
\end{equation}
\end{comment}

\begin{equation}
B \geq  C_1 \frac{1}{\alpha^2 L^2}, \quad D_{in}, BD_o \geq C_2 \frac{\tsigma^2}{\alpha^2 \sigma^2 L^2},
\end{equation}
\sloppy for some constants $C_1$ and $C_2$,
then FO-MAML finds a point $w^{\dag}$ satisfying the condition $\E[\|\nabla F(w^{\dag})\|]\leq \mathcal{O}(\alpha \sigma L)$,  after at most 
$\Delta \bigO({1}/{(\alpha^2 \sigma^2 L)})$ iterations.
\end{corollary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Convex Quadratic Case}\label{Qudratic_MAML}
Theorem \ref{First_order_MAML_det_simple} suggests that FO-MAML might not be able to achieve any arbitrary level of accuracy, even when exact gradients and Hessians are available. In this subsection, we provide an example to show that this is indeed the case. In particular, we consider the case that we have $n$ equally likely tasks, where the loss function corresponding to task $i$ is given by 
\begin{equation}
f_i(w) = \frac{1}{2} w^\top A_i w + b_i^\top w + c_i	
\end{equation} 
where $c_i \in \R$, $b_i \in \R^d$, , and $A_i \in \R^{d \times d}$ is a symmetric and positive definite matrix with $\|A_i\| \leq L$. Note that, in this case, we have
\begin{equation}
\nabla f_i(w) = A_i w + b_i, \quad \nabla^2 f_i(w) = A_i. 	
\end{equation}
Also, throughout this section, we assume we have access to the exact value of Hessians and gradients, and also we go over all tasks at each iteration, i.e., $\B_k$ is equal to the set of all tasks. We further assume $\alpha < 1/L$. 


\vspace{2mm}

\noindent $\bullet$ \textbf{Solution of MAML Problem}

Let us first derive the solution to problem \eqref{main_prob}. Setting $\nabla F(w^*)$ equal to $0$ implies that
\begin{equation}
\frac{1}{n} \sum_{i=1}^n (I - \alpha A_i) \left ( A_i \left (w^* - \alpha (A_i w^* + b_i) \right ) + b_i\right ) = 0.
\end{equation}
Simplifying this equation yields
\begin{equation}\label{w_MAML_quad}
\left ( \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i)^2 A_i \right ) w^* = - \left ( \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i)^2 b_i \right ).	
\end{equation}
Note that, for any $i$, $(I - \alpha A_i)^2 A_i$ is positive definite. This is due to the fact that, for any $u \in \R^d$, we have
\begin{align*}
u^\top 	(I - \alpha A_i)^2 A_i u = \left ( (I - \alpha A_i) u \right )^\top A_i \left ( (I - \alpha A_i) u \right ) > 0
\end{align*}
where the first equality follows from the fact that $A_i$ is symmetric and the last inequality is obtained using positive definiteness of $A_i$. As a result, and since sum of positive definite matrices is also positive definite, $\left ( \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i)^2 A_i \right )$ is positive definite, and hence invertible. Thus, from \eqref{w_MAML_quad}, we have
\begin{equation}\label{w_MAML_quad_2}
w^* = 	- \left ( \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i)^2 A_i \right )^{-1} \left ( \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i)^2 b_i \right ).
\end{equation}

\vspace{2mm}

\noindent $\bullet$ \textbf{What FO-MAML Converges to?}

FO-MAML update is given by
\begin{align}\label{w_FOMAML_quad}
w_{k+1} &= w_k - \alpha 	\frac{1}{n} \sum_{i=1}^n \left ( A_i \left (w_k - \alpha (A_i w_k + b_i) \right ) + b_i\right ) \nonumber\\
& = \left ( I - \alpha \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i) A_i \right ) w_k - \alpha \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i) b_i.
\end{align}
Note that, since $\alpha < 1/L$, for any $i$, $I-\alpha A_i$ is symmetric and positive definite. Note that since both $I-\alpha A_i$ and $A_i$ are positive definite and $(I-\alpha A_i)A_i$ can be written as $A_i^{1/2} (I-\alpha A_i) A_i^{1/2}$, then we can show that $(I-\alpha A_i)A_i$ is also positive definite. In addition, since $\|A_i\| \leq L$ and $\|I - \alpha A_i\| \leq 1$, we have $\| (I-\alpha A_i)A_i\| \leq L$. Therefore, the term $\frac{1}{n} \sum_{i=1}^n (I - \alpha A_i) A_i$ is  positive definite and its norm is upper bounded by $L$. Since $\alpha < 1/L$, this implies that $I - \alpha \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i) A_i$ is positive definite, and thus invertible.

Using this result, it is immediate to see $\{w_k\}_k$ \eqref{w_FOMAML_quad} converges to
\begin{equation}\label{w_FOMAML_quad_2}
w_{FO} = - \left ( \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i) A_i \right )^{-1} \left ( \frac{1}{n} \sum_{i=1}^n (I - \alpha A_i) b_i \right ).	
\end{equation}
Comparing \eqref{w_MAML_quad_2} and \eqref{w_FOMAML_quad_2}, it is clear that FO-MAML does not converge to the solution of MAML problem denoted by $w^*$. However, if either $\alpha$ is very small or if $A_i$ are all close to some $A$ and $b_i$ are all close to some $b$ which leads to $\sigma$ being very small, then $w_{FO}$ would be very close to $w^*$, which is in line with what we observed in Theorem \ref{First_order_MAML_det_simple}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% S E C T I ON  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Convergence of HF-MAML}



Now we proceed to analyze the overall complexity of our proposed HF-MAML method.
\begin{theorem}\label{Thm_HF_MAML_simple}
%%%
Consider the function $F$ defined in \eqref{main_prob} for the case that $\al \in (0,\frac{1}{6L}]$. Suppose Assumptions~\ref{ass:boundedness}-\ref{asm_simplify} hold. Consider running HF-MAML with batch sizes satisfying the conditions $D_h \geq \ceil{36 (\al \rho \tsigma)^2}$ and $B \geq 20$.
Let $\beta_k = \tilde{\beta}(w_k)/25$
where $\tilde{\beta}(w)$ is defined in \eqref{beta_update}. Also, we choose the approximation parameter $\delta_k^i$ in HF-MAML as

\begin{equation*}
\delta_k^i = \frac{1}{6 \rho \alpha \| \tilde{\nabla} f_i(w_k\!-\!\al \tilde{\nabla} f_i(w_k,\D_{in}^i),\D_{o}^i) \|}.
\end{equation*}
Then, HF-MAML finds a solution $w_\eps$ such that
%%%%

\begin{equation}
 \E[ \| \nabla F(w_\eps) \|] \leq \bigO \bigg( \sqrt{\frac{\sigma^2}{B} + \frac{\tsigma^2}{B D_o} + \frac{\tsigma^2}{D_{in}}} \bigg) + \eps	
\end{equation}
with a total number of iterations of

\begin{equation}
\bigO(1) \Delta \min \left \{ \frac{L}{\eps^2},
\frac{LB}{\sigma^2} + \frac{L(B D_o+D_{in})}{\tsigma^2} \right \} .
\end{equation}
%iterations, where $\Delta:= (F(w_0) - \min_{w \in \R^d} F(w) )$.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%
%\begin{proof}
%Check Appendix \ref{Thm_HF_MAML_proof} for the general statement of the theorem and its proof.
%\end{proof}


Comparing the results in Theorem~\ref{Thm_HF_MAML_simple} for HF-MAML with the result in Theorem~\ref{Thm_SGD_general_simple} for MAML shows that the complexity of these methods and the resulted accuracy are the same, up to a constant factor. Hence, HF-MAML recovers the complexity of MAML \textit{without} computing second-order information or performing any update that has a complexity of $\mathcal{O}(d^2)$. %As the results for HF-MAML are similar to the ones for MAML, we can show that similar results to the ones in Corollary~\ref{cor_large_batch_MAML} also hold for HF-MAML (Appendix~\ref{Thm_HF_MAML_proof}).
Also, as stated after Theorem \ref{Thm_HF_MAML_simple}, the following result holds as an immediate consequence:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%       COROLLARY       %%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{corollary}\label{cor_large_batch_HF_MAML}
Suppose the condition in Theorem~\ref{Thm_HF_MAML_simple} are satisfied. Then, if the batch sizes $B$, $D_o$, and $D_{in}$ satisfy the following conditions, 
%%%
\begin{equation*}
B \geq  C_1 \frac{\sigma^2}{\eps^2}, \quad D_{in}, BD_o \geq C_2 \frac{\tsigma^2}{\eps^2},
\end{equation*}
for some constants $C_1$ and $C_2$, then the iterates generated by HF-MAML finds an $\eps$-FOSP, i.e., $\E[\|\nabla F(w)\|]\leq \eps$,  after $\Delta \bigO ({L}/{\eps^2})$ iterations.
\end{corollary}
%\begin{remark}
%MAML and HF-MAML find an $\epsilon$-FOSP after $\bigO(1/\epsilon^{2})$ iterations with $\bigO(1/\epsilon^{4})$ samples per iteration which means $\bigO(1/\epsilon^6)$ total sample complexity. This is different from classic nonconvex results where, for instance, Natasha 2 \citep{Natasha2}, finds an $\epsilon$-FOSP using $\bigO(1/\epsilon^{3.25}) $ samples. However, note that the latter has one source of randomness, while MAML includes two sources (tasks and data corresponding to tasks). By only considering one source of randomness, total sample complexity of MAML and HF-MAML is $\bigO(1/\epsilon^ 4)$ which is close to Natasha 2 but not stronger. Indeed, this complexity can be improved using variance reduction techniques. 
%\end{remark}

